What Is Near?: Room Locality Learning for Enhanced Robot Vision-Language-Navigation in Indoor Living Environments

Humans use their knowledge of common house layouts obtained from previous experiences to predict nearby rooms while navigating in new environments. This greatly helps them navigate previously unseen environments and locate their target room. To provide layout prior knowledge to navigational agents based on common human living spaces, we propose WIN (\textit{W}hat \textit{I}s \textit{N}ear), a commonsense learning model for Vision Language Navigation (VLN) tasks. VLN requires an agent to traverse indoor environments based on descriptive navigational instructions. Unlike existing layout learning works, WIN predicts the local neighborhood map based on prior knowledge of living spaces and current observation, operating on an imagined global map of the entire environment. The model infers neighborhood regions based on visual cues of current observations, navigational history, and layout common sense. We show that local-global planning based on locality knowledge and predicting the indoor layout allows the agent to efficiently select the appropriate action. Specifically, we devised a cross-modal transformer that utilizes this locality prior for decision-making in addition to visual inputs and instructions. Experimental results show that locality learning using WIN provides better generalizability compared to classical VLN agents in unseen environments. Our model performs favorably on standard VLN metrics, with Success Rate 68\% and Success weighted by Path Length 63\% in unseen environments.

==> sections/appedix.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
In this work, we present a novel approach for VLN based on using topological knowledge to predict neighbouring rooms in domestic environments. Our modular \winmodel~model demonstrates a significant performance gain in unseen environments compared to a simple and state-of-the-art baseline. In summary, we encode topological patterns commonly found in indoor environments using a prediction model and use this knowledge to assist Vision-language Navigation agents in making action decisions at each time step. Empirical results on the Room-to-Room dataset show that the \winmodel~method outperforms both simple and SoTA baseline methods while reducing the SR margin between seen and unseen environments. A potential extension of this work is to learn general topological relationships from house plan datasets such as CubiCasa5k \cite{Kalervo2019cubicasa} and semantic relations from commonsense knowledge bases. 

